Assessing the Students' Understanding and their Mistakes in Code Review Checklists -- An Experience Report of 1,791 Code Review Checklist Questions from 394 Students

Code review is a widely-used practice in software development companies to identify defects. Hence, code review has been included in many software engineering curricula at universities worldwide. However, teaching code review is still a challenging task because the code review effectiveness depends on the code reading and analytical skills of a reviewer. While several studies have investigated the code reading techniques that students should use to find defects during code review, little has focused on a learning activity that involves analytical skills. Indeed, developing a code review checklist should stimulate students to develop their analytical skills to anticipate potential issues (i.e., software defects). Yet, it is unclear whether students can anticipate potential issues given their limited experience in software development (programming, testing, etc.). We perform a qualitative analysis to investigate whether students are capable of creating code review checklists, and if the checklists can be used to guide reviewers to find defects. In addition, we identify common mistakes that students make when developing a code review checklist. Our results show that while there are some misconceptions among students about the purpose of code review, students are able to anticipate potential defects and create a relatively good code review checklist. Hence, our results lead us to conclude that developing a code review checklist can be a part of the learning activities for code review in order to scaffold students' skills.

==> Makefile <==
FILE_NAME := paper

TEMP_FILES := \
	$(FILE_NAME).aux \
	$(FILE_NAME).bbl \
	$(FILE_NAME).log \
	$(FILE_NAME).blg \
	$(FILE_NAME).brf \
	$(FILE_NAME).out

SECTION_FILES = \
	paper.tex \
	sections/defect_type.tex \

BIBTEX_FILES = \
	filteredref.bib 

GEN_FIGURES = \
	$(NULL)

# STATIC_FIGURES = \
# 	figure/overview.pdf 

DEBUG=no
ifneq '$(DEBUG)' 'yes'
LATEX_FLAGS="-interaction=batchmode"
endif

.DELETE_ON_ERROR:

################################################################################
# Main paper building
################################################################################
# $(STATIC_FIGURES)
$(FILE_NAME).pdf: $(SECTION_FILES) $(GEN_FIGURES) $(BIBTEX_FILES) 
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	bibtex $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	rm -f $(TEMP_FILES)
	# open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf


################################################################################
# Camera-Ready
################################################################################
.PHONY: camera
camera: 
	pdftops $(FILE_NAME).pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $(FILE_NAME).pdf $(FILE_NAME)-new.pdf
	# pdffont $(FILE_NAME).pdf
	mv $(FILE_NAME)-new.pdf $(FILE_NAME).pdf
	# open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf
	
################################################################################
# Figures
################################################################################

#$(GEN_FIGURES): %.pdf: scripts/rms/analysis_figures.r scripts/rms/util.r
#	Rscript $<

################################################################################
# Clean
################################################################################
.PHONY: clean
clean:
	rm -f $(TEMP_FILES) $(GEN_FIGURES) $(FILE_NAME).pdf


==> sections/defect_type_large.tex <==

\begin{table}[t]
\caption{A Taxonomy of Defects in Code Review~\cite{mantyla2008types}}
\label{Table:taxonomy}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llp{12.5cm}} 
\hline
Defect Type & Sub-type & Description \\
\hline
Documentation & Naming & Defects on the software element (methods, variables, etc.) names such as uninformative names or names that violate the standard convention. \\
& Comment & Defects on a code comment such as a lack of comments, comments that violate the standard convention. \\
& Debug Info & Defects on the information that will be used for debugging such as uninformative exception message. \\
& Element Type & Defects on the type of variables such as an undefined type in Python since it may cause a confusion of using variable. \\
& Immutable & defect types on not declaring variable to be immutable when it should have been.\\
& Visibility & Defects on the visbility of variables, for example, should this variable be a global variable. \\
& Other Textual Defects & Other defects relating to textual information.\\
\hline
Visual Representation & Defects on the bracket Usage & defect types on incorrect or missing necessary brackets. \\
& Indentation & Defects on incorrect indentation. \\
& The Blank Line Usage & Defects on the use of incorrect or unnecessary blank lines. \\
& Long Line & Defects on a long code statement which cause the readability. \\
& Space Usage & Defects on unnecessary blank spaces. \\
& Grouping & Defects on the cohesion of code elements, for example, variables should be introduced closely to the related method. \\
\hline
Structure
& Long Sub-routine &  Defects on a lengthy function or procedure. \\
& Dead Code & Defects on code statements that are not executed or used or executed but do not serve any meaningful purpose. \\
& Duplication & Defects on exact repeated or duplicate code statements. \\
& Semantic Duplication & Defects on code redundancy, i.e., code statements are dissimilar but serve similar purposes. The concern also includes replacing source code with an existing library. \\
& Complex Code & Defects on source code that are difficult to comprehend. \\
& Consistency & Defects on the ways of implementation should be in a similar fashion.\\
& New Functionality & Defects on a piece of source code that does not have a single purpose and it requires a new function. \\
& Use Standard Method & Defects whether the standardised approach of implementation should be used. \\
& Other & Other defects related to  refactoring, organising, and improving source code.\\
\hline
Resource
& Variable Initialisation & Defects on the variables that are left uninitialised or incorrectly initialised. \\
& Memory Management & Defects on how program use and manage the memory. \\
& Data \& Resource Manipulation & Other defects relating to managing other related resources such as files. \\
\hline
Check
& Check Function & Defects on a value returned from a function. \\
& Check Variable & Defects about whether the program validate the variable values. This includes the parameter variables, loop control variables.\\
& Check User Input & Defects on the validity of user input. \\
\hline
Interface
& Parameter & Defects on incorrect or missing parameters when calling another function or library. \\
& Function Call & Defects on incorrect interaction between a function and another part of the system or class library.\\
\hline
Logic
& Compare & Defects on logic for a comparison. \\
& Compute & Defects on incorrect logic when the system runs. \\
& Wrong Location & Defects on the wrong location of the operation although it is correct. \\
& Algorithm/Performance & Defects on the efficiency of the algorithm.\\
& Other & Other defects related to the correctness or existence of logic.\\
\hline
Large Defects 
& GUI & Defects about the completeness and correctness of user interfaces. \\
& Completeness & Defects about whether the implementation is complete.\\
\hline
\end{tabular}
}
\end{table}
